Rank-Regret Minimization

Multi-criteria decision-making often requires finding a small representative set from the database. A recently proposed method is the regret minimization set (RMS) query. RMS returns a size $r$ subset $S$ of dataset $D$ that minimizes the regret-ratio (the difference between the score of top-1 in $S$ and the score of top-1 in $D$, for any possible utility function). RMS is not shift invariant, causing inconsistency in results. Further, existing work showed that the regret-ratio is often a made-up number and users may mistake its absolute value. Instead, users do understand the notion of rank. Thus it considered the problem of finding the minimal set $S$ with a rank-regret (the rank of top-1 tuple of $S$ in the sorted list of $D$) at most $k$, called the rank-regret representative (RRR) problem. Corresponding to RMS, we focus on the min-error version of RRR, called the rank-regret minimization (RRM) problem, which finds a size $r$ set to minimize the maximum rank-regret for all utility functions. Further, we generalize RRM and propose the restricted RRM (i.e., RRRM) problem to optimize the rank-regret for functions restricted in a given space. Previous studies on both RMS and RRR did not consider the restricted function space. The solution for RRRM usually has a lower regret level and can better serve the specific preferences of some users. Note that RRM and RRRM are shift invariant. In 2D space, we design a dynamic programming algorithm 2DRRM to return the optimal solution for RRM. In HD space, we propose an algorithm HDRRM that introduces a double approximation guarantee on rank-regret. Both 2DRRM and HDRRM are applicable for RRRM. Extensive experiments on the synthetic and real datasets verify the efficiency and effectiveness of our algorithms. In particular, HDRRM always has the best output quality in experiments.

==> file/response.tex <==
\section*{Response to Reviewer Comments}
The reviewers have given us many helpful comments. We are grateful to have the opportunity to promote our paper under the guidance of these comments. Overall, the major changes of the paper are summarized as follows:

\begin{enumerate}
	\item The expression of this paper has been polished to improve the readability.
	\item We rewrite the flaws of the regret-ratio and RMS\cite{nanongkai2010regret} problem in Section \ref{s_intro}. 
	\item We clarify the flaws of the dual problem RRR\cite{asudeh2019rrr} in Section \ref{s_def}. 
	\item We prove that RRM and RRRM are scale invariant (the optimum result remains the same after adding an arbitrary non-negative $d$-dimensional vector to all tuples) in Section \ref{s_theoretical}. 
	\item We have updated the time complexity of HDRRM, MDRRR and MDRRR$_r$, and show their space complexity in Section \ref{s_intro} and \ref{s_hd}. 
	\item We give an example in Section \ref{s_def} to show that minimizing regret-ratio\cite{nanongkai2010regret} does not typically minimize rank-regret.
	\item We give an example in Section \ref{s_2d} to illustrate the process of handling intersections in 2DRRM.
	\item We add experiments to compare our algorithm HDRRM with the MDRMS\cite{asudeh2017efficient} algorithm for RMS.
	\item Besides, some subsections are reformed in response to the requirements of reviewers.
\end{enumerate}

Thanks for pointing out the typos and the grammar errors in detail. We apologize for the inconvenience caused to the reviewers by our poor expression. We receive the comments from Reviewer \#1, Reviewer \#2, and Reviewer \#5.  The detailed responses for all these comments are listed one by one as follows. 

\subsection*{To Reviewer \#1}

\noindent{\bf O1.}
While the authors compare extensively against the dual approach which is then translated to their problem via binary search, they do not compare sufficiently against RMS approaches that optimize the regret, both conceptually and experimentally. It is not clear to me why the optimal solutions to the 2 problems would be different. What is a minimal example that illustrates this? And it would make more sense to compare against these algorithms in the experimental section, e.g. from reference \cite{xie2018efficient}.

\noindent{\color{purple}{\bf Reply:}
	Thanks for careful reviewing. The comparison of RRM and RMS\cite{nanongkai2010regret} approaches are indeed not fully considered in the original paper. Based on the comment, we handle it as follows. 
	
	First, in the fourth-to-last paragraph of Section \ref{s_def}, we add an example shown in Table \ref{tab_example}. When $r=1$, the optimal solutions of the 2 problems are different but close. To magnify the difference, we shift the second attribute $A_2$ and get a new dataset shown in Figure \ref{fig-shift}. The updated values on $A_2$ are in the top range. RMS pursues approximations on the absolute utility (i.e., regret-ratio) and directly ignores $A_2$. After shifting, the solution of RMS changes drastically and has the worst rank-regret. In contrast, the solution of RRM remains the same. Minimizing regret-ratio does not typically minimize rank-regret. It is shown that RMS is not shift invariant (i.e., if we add a fixed constant to all values in some attribute, RMS may change the result). We prove in Section \ref{s_theoretical} that RRM is shift invariant.
	
	In addition, following the settings in \cite{asudeh2019rrr}, we add experiments to compare our algorithm HDRRM against the MDRMS\cite{asudeh2017efficient} algorithm designed for RMS. In experiments, HDRRM always has the lowest rank-regret. Correspondingly, MDRMS sometimes has the highest rank-regret which is more than one order of magnitude larger. Due to time and space constraints, we do not make comparisons with other RMS approaches. If possible, we will supplement it in the future. 
}

\noindent{\bf O2.}
I do not really understand why it is important for the present paper that "the regret-ratio cannot accurately quantify the “regret” level of users." The algorithms in this paper or the works on RMS queries do not take the regret as an input--they try to minimize it internally. Thus, the users only have to provide the desired size.

\noindent{\color{purple}{\bf Reply:}
	Thanks for the comment. Our description in the original paper does not fully reflect the difference between RRM and RMS queries. Sorry to confuse the reviewers, we revise it in Section \ref{s_intro} and \ref{s_def}. 
	
	Though both queries return a set with the desired size, their optimization goals are different (rank-regret and regret-ratio). Tuples in a dataset are usually not uniformly distributed by utility, and RMS pursues approximations on the absolute utility (i.e., regret-ratio), possibly resulting in a significant increase on rank-regret as shown in Figure \ref{fig-shift}. Minimizing regret-ratio does not typically minimize rank-regret. The optimal solutions to the 2 queries are different.
	
	Further, RRM is shift invariant, but RMS is not. The solution of RRM remains the same after shifting, and that of RMS may change. In Section \ref{s_intro}, we add  several examples show that shift variance causes inconsistency. 
	
	In addition, the utility/regret-ratio is usually an artificial number with no direct significance, and users may not understand its absolute value. We add two examples in Section \ref{s_intro} to introduce it. In contrast, users do understand the notion of rank. Both are "regret", but users can better understand the rank-regret. 
}

\noindent{\bf O3.}
Several ideas of the presented algorithms are not new given the extensive literature and could be considered incremental.

\noindent{\color{purple}{\bf Reply:}
	Thanks for careful reviewing. Compared to the related works, the ideas of our algorithms can indeed be considered incremental. However, both algorithms in the paper can be applied to the restricted function space, which is not considered by the previous. In addition, the 2D algorithm returns the optimal solution for RRM, and can be transformed into an exact algorithm for RRR\cite{asudeh2019rrr}.
}

\noindent{\bf O4.}
How is it possible that the number of dimensions does not appear in the running time of HDRRM? What if, for example, $d>n$?

\noindent{\color{purple}{\bf Reply:}
	Thanks for the comment. The impact of dimension on the time complexity is indeed a very interesting question. In the first paragraph of Section \ref{s_def}, we add an assumption that the number of attributes is a fixed constant, which is reasonable in many scenarios and appears in many related works (e.g., \cite{asudeh2017efficient, asudeh2019rrr, xie2018efficient, xie2020being, xie2020experimental}). In Theorem \ref{t_RRM_time}, we show the time and space complexity of HDRRM related to $d$. Similarly, we also modify the time and space complexity of MDRRR and MDRRR$_r$. If possible, we would like to design an algorithm in the future which has a time complexity linear with $d$.
}

\noindent{\bf O5.}
Related to O1, is the difference between the lower bound given in Sec \ref{s_lower_bound} (compared to the RMS algorithms) just the difference in scale ($[1,n]$ instead of $[0,1]$)? Or is there some difference in hardness?

\noindent{\color{purple}{\bf Reply:}
	Thanks for the comment, which is really a question worth exploring. Though the lower-bound $\Omega(n/r)$ given in Sec \ref{s_lower_bound} is inspired by that for the regret-ratio in \cite{nanongkai2010regret}, the difference between them is not just the difference in scale ($[1,n]$ for rank-regret and $[0,1]$ for regret-ratio). When $d=2$, multiplying $\Omega(r^{-2/(d-1)})$ (the bound for regret-ratio) by $n$ results in a looser lower-bound $\Omega(n/r^2)$. In addition, we would like to give a strong bound related to $d$ for RRM in the future.
}

\noindent{\bf O6.}
It would be good to mention something about how the algorithms of this paper compare against other in space consumption. For example in Table \ref{tab_compare}, or in the experimental section, even as a short sentence if there is no space for other figures.

\noindent{\color{purple}{\bf Reply:}
	Thanks for the comment, which is really a good suggestion. As far as we know, all related researches basically do not take space complexity into consideration. In Theorem \ref{t_RRM_time}, we show the space complexity of HDRRM. In Sec \ref{s_intro} and \ref{s_hd_com}, we also supplement the space complexity of MDRRR and MDRRR$_r$, which are obviously worse than that of HDRRM. For time and space constraints, we do not make a comparison on space consumption in experiments. %We would like to fulfill it in the future.
}

\noindent{\bf O7.}
The presentation in several places is lacking and makes the paper hard to understand.

\noindent- Page 2 "but a rank-regret of $2k$". I imagine this means that $k$ is the optimal rank-regret and the algorithm achieves up to $2k$.

\noindent{\color{purple}{\bf Reply:}
	Sorry to confuse you, we make a detail declaration in the refined version. 2DRRR is an approximation algorithm for the RRR\cite{asudeh2019rrr} problem. Given a threshold $k$, RRR aims to find the minimum set with a rank-regret at most $k$. 2DRRR returns a set with size and rank-regret at most $r_k$ and $2k$ respectively, where $r_k$ is the minimal size of sets with rank-regrets at most $k$.
}

\noindent- Page 2 "bounds the output...size sets". The properties of HDRRM are very unclear from this sentence (it also appears elsewhere). What is a "double guarantee" and why do the sets have this size, isn't the size fixed as an input?

\noindent{\color{purple}{\bf Reply:}
	We are sorry to confuse you with our poor writing. In the revision, we rewrite all descriptions about the theoretical guarantees of HDRRM. HDRRM is an algorithm for RRM that returns a size $r$ set and approximates the minimal rank-regret for any $O(\frac{r}{\ln\ln n})$ size set. Further, "double guarantee" is about the output rank-regret of HDRRM and describes the second and third clauses of Theorem \ref{t_RRM_quality}.
}

\noindent- Page 3 "excellent upper bound". This is very ambiguous.

\noindent{\color{purple}{\bf Reply:}
	Sorry for the ambiguous description. We revise it to make it clear in the first paragraph of Section \ref{s_theoretical}, i.e., "an upper-bound guarantee independent of the data size."
}

\noindent- Page 4 "Algorithms proposed...experiments". That is not the case, e.g., in Figure \ref{ex-indep-n-tr} the rank-regret increases.

\noindent\noindent{\color{purple}{\bf Reply:}
	Thanks for pointing out the mistake. Based on the comment, we fix it in Section \ref{s_lower_bound}. 
}

\noindent- Fig 3: Shouldn't $t_5$ and $t_6$ be aligned to some other tuples?

\noindent{\color{purple}{\bf Reply:}
	Thanks for pointing out our mistake. We fix it in Figure \ref{fig-example} and Figure \ref{fig-shift}.
}

\noindent- Some experiments such as Fig. \ref{ex-2d-n-t} are hard to read. Maybe consider replacing them with barplots with fewer points?

\noindent{\color{purple}{\bf Reply:}
	Thanks for your helpful advice. We turn both Figures \ref{ex-2d-n-t} and \ref{ex-2d-r-t} into bar charts in the revision.
}

\noindent- Page 10: "equal to $O(r\ln n/\delta^2)$": how can it be equal to a big-O? Do the authors mean that they set it exactly to that value?

\noindent{\color{purple}{\bf Reply:}
	We are sorry for not clearly stating the value. We have added the specific expression in the first paragraph of Section \ref{s_ex_hd}.
}

\noindent- Page 12: "1610!": The exclamation mark here is unnecessary and makes it look like a factorial.

\noindent{\color{purple}{\bf Reply:}
	Thanks for your careful reviewing. We have fixed it in the revision.
}

\subsection*{To Reviewer \#2}
\noindent{\bf O1.}
It may be incremental (especially with respect to citation \cite{asudeh2019rrr}).

\noindent{\color{purple}{\bf Reply:}
Thanks for the comment. Due to studying a dual version of RRR\cite{asudeh2019rrr}, this paper can indeed be considered incremental. However, there are many innovations in our work. Firstly, we generalize the problem and restrict the function space, which is not considered in the previous studies. Secondly, we propose a 2D algorithm that returns the optimal solution. The algorithm can be transformed into an exact algorithm for RRR\cite{asudeh2019rrr}, which is a huge breakthrough. Thirdly, we prove some theoretical properties of the problem (e.g., the shift invariance, lower-bound, and candidate tuples). 
}

\noindent{\bf O2.}
The problem examined in \cite{asudeh2019rrr} seems more natural to me for the following reason:

The problem in this paper is: find a representative set of size $r$ that minimizes the maximum rank-regret. The problem in \cite{asudeh2019rrr} is: given a rank-regret threshold $k$, find the minimum set with a maximum rank-regret at most $k$.

I find the problem in \cite{asudeh2019rrr} more natural because the user is interested above all in a reasonable rank-regret threshold. If the set for a reasonable rank-regret is too large then, we may want to solve the problem in the present paper but we may get an unsatisfactory result in that the maximum rank-regret may be too high to be of any use in decision-making.

\noindent{\color{purple}{\bf Reply:}
	Thanks for the comment, which is indeed what we do not explain clearly in the original paper. We clarify it in the third-to-last and second-to-last paragraph of Section \ref{s_def}. Depending on the search needs of users, different versions of queries (RRM in the paper and RRR in \cite{asudeh2019rrr}) can be applied. 
	
	Specifying the output size is critical due to some considerations such as the website display size, upload speed to the cloud and communication bandwidth between hosts. The output size represents the effort required by the user to make a decision. RRR cannot directly control the output size and may return a huge set. Users may be unable or unwilling to browse thousands of tuples. A large representative set provides little help for the user to make a decision. Therefore, we usually would like to return only a limited number $r$ of tuples.
	
	The scenario in the comment (i.e., the rank-regret may be too high to be of any use) should be rare. As shown in experiments, RRM has a solution with a small rank-regret in most cases. Further, a high rank-regret is usually due to a huge dataset. The range of rank-regret is $[1,n]$. For datasets of different sizes, the same rank-regret has different practical meanings. Similar to regret-ratio, we can normalize the range to $[0,1]$ (i.e., divide rank-regrets by $n$) and equivalently use percentages to represent user regret. Expressing rank in the form of percentage is much common. In experiments of \cite{asudeh2019rrr}, the input rank-regret threshold is also represented by a percentage (e.g., top-1\%). In addition, our algorithms can be applied to RRR\cite{asudeh2019rrr} with simple modifications.
}

\subsection*{To Reviewer \#5}

\noindent{\bf O1.}
The motivation of the studied problem RRM is not enough. The introduction only mentions a website example. It would be better to discuss the weakness of the problem proposed by \cite{asudeh2019rrr} and present more real-life examples.

\noindent{\color{purple}{\bf Reply:}
	Thanks for careful reviewing. The weakness of RRR\cite{asudeh2019rrr} is indeed not fully expressed in the original paper. We clarify it in the third-to-last paragraph of Section \ref{s_def}. We present more real-life examples in the introduction to show that specifying the output size is critical (the website display size, upload speed to the cloud and communication bandwidth between hosts). 
	
	RRR aims to find the minimum set that fulfill a given rank-regret threshold. RRR cannot directly control the output size and may return a huge set. The output size represents the effort required by the user to make a decision. Users may be unable or unwilling to browse thousands of tuples. A large representative set provides little help for the user to make a decision. Therefore, compared to RRR\cite{asudeh2019rrr}, we would like to choose RRM. 
}

\noindent{\bf O2.}
The introduction section discusses the regret ratio problem. It is hard to see why there is a problem. This paper claims that "It indicates that more than half of wines approximate the top-1 based on regret-ratio, better than they actually do". If this is the case, then half of the wines in the dataset are good and should not be regretful for users to choose. It is reasonable.

\noindent{\color{purple}{\bf Reply:}
	Thanks for the comment. Our description in the original paper does not fully reflect the drawbacks of the regret-ratio and RMS\cite{nanongkai2010regret}. Sorry to confuse the reviewers, we revise it in Section \ref{s_intro}. We have discarded the ambiguous example in the original paper.
	
	First, RMS is not shift invariant (i.e., if we add a fixed constant to all values in some attribute, RMS may change the result), which causes inconsistency in outputs. For example, temperatures have to be shifted when converting between scales (°C, °F, and K). After shifting, the dataset is essentially unchanged and query results should be the same. Paradoxically, RMS may have different outputs. Similar examples are spatial coordinates and altitudes. In addition, some presuppositions of RMS also require data shifting. 
	
	Second, the utility/regret-ratio is usually an artificial number with no direct significance, and users may not understand its absolute value. We add two examples in Section \ref{s_intro} to introduce it. Further, a small range in regret-ratio can include a large fraction of dataset.
}


\noindent{\bf O3.}
This paper should discuss more of the related work. As mentioned in the introduction, the regret-ratio minimization problem is closely related to the topic studied in this paper. Some examples are \cite{cao2017k,nanongkai2010regret,xie2018efficient}. They find a set of r tuples that fulfill the regret ratio requirement. There should be a discussion of why the algorithms \cite{cao2017k,nanongkai2010regret,xie2018efficient} cannot be adapted to the RRM problem.

\noindent{\color{purple}{\bf Reply:}
	Thanks for the comment, which is indeed what we do not fully explain in the original paper. We clarify it in the fourth-to-last of Section \ref{s_def}. And we add experiments to compare our algorithm HDRRM with the MDRMS\cite{asudeh2017efficient} algorithm designed for the regret-ratio minimization set (RMS) problem.
	
	Though both problems aim to return a set with the desired size, their optimization goals are different (rank-regret and regret-ratio). The optimal solutions to the 2 problems are different. Since tuples in a dataset are usually not uniformly distributed by utility, minimizing regret-ratio does not typically minimize rank-regret. Thus the algorithms for RMS cannot be adapted to RRM. We add an example in Figure \ref{fig-shift} to illustrate this. The RMS problem pursues approximations on the absolute utility (i.e., regret-ratio), possibly resulting in a significant increase on rank-regret. If the values on a attribute are in the top range, RMS will directly ignore the attribute but RRM will not. In addition, the algorithms for RMS did not consider the restricted function space.
	
	Further, RRM is shift invariant, but RMS is not. The optimal solution of RRM remains the same after shifting, and that of RMS may change. In Section \ref{s_intro}, we add several examples show that shift variance causes inconsistency.
}

\noindent{\bf O4.}
Theorem 3 discusses the input of problem RRM and the convex hull. It is unclear how this theorem helps illustrate the rest of the paper.

\noindent{\color{purple}{\bf Reply:}
	Thanks for the comment, which is really a question. Indeed, the theorem about the convex hull helps little for the the rest of paper. Thus, we have removed it in the revised version. 
}

\noindent{\bf O5.}
The description of the algorithm needs to be improved. There are some parts which have difficulties for reading. Some parts are listed as follows.

\noindent E.g., Section \ref{s_2d_pre} discusses the convex chain. It mentions that "S and the corresponding chain C(S) have the same size.". What if $S = \{t_2, t_3, t_4\}$?

\noindent{\color{purple}{\bf Reply:}
	Thanks for pointing out the mistake. Based on the comment, we fix it in Section \ref{s_2d_pre}. 
}

\noindent E.g., In Min-Heap $H$, it mentions "$l_5$ and $l_7$ become immediate neighbors for the first time". How to learn it is the first time?

\noindent{\color{purple}{\bf Reply:}
	We are sorry for not clearly stating it. We have made a detail declaration in the refined version. $H$ is implemented by a binary search tree. If the intersection $(l_5, l_7)$ lies between $\mathcal{L}$ and $x=1$ (i.e., not processed) and is not in $H$ (i.e., not inserted), then $l_5$ and $l_7$ become immediate neighbors for the first time. 
}

\noindent E.g., The description of matrix $M$ is unclear. It would be better to give a detailed example for the case when $l_i$ and $l_j$ are skyline lines. It is not readable to just show different colors of dots.

\noindent{\color{purple}{\bf Reply:}
	We are sorry to confuse you with our poor writing. We add a paragraph with Table \ref{tab_m} in Section \ref{s-2d-ad} to briefly illustrate the process of handling intersections. 
	
}

\noindent E.g., Section \ref{s_hd} presents the way of sampling utility vectors. There should be an intuition illustration why the algorithm samples the utility vectors in this way. Besides, it would be better to give an example for $\mathbb{D}_b$ (e.g. a figure similar to Figure \ref{fig-sphere}).

\noindent{\color{purple}{\bf Reply:}
	We realize that our presentation needs to be improved. Thanks to the patience of reviewers for pointing out what are unclear in the original paper. we have made detail declarations in the revision. $\mathbb{D}_a$ is the uniform sample set of $\mathbb{S}$ to estimate the area of some subregions of $\mathbb{S}$ (e.g., $\cup_{t\in S} V_\mathbb{S}(t)$). $\mathbb{D}_b$ is used to guarantee that for any $u\in\mathbb{S}$, there is a $v\in\mathbb{D}_b$ close to $u$. We give an example for $\mathbb{D}_b$ in Figure \ref{fig-polar}. 
}

\noindent{\bf O6.}
The regret-ratio minimization problem is closely related to the problem studied in the paper. The experiments need to include algorithms for regret-ratio minimization problem. It is important to present that the proposed algorithm is better than the regret-ratio minimization algorithms under the rank-regret measurement.

\noindent{\color{purple}{\bf Reply:}
	Thanks for the comment, which is really a good suggestion. Following the settings in \cite{asudeh2019rrr}, we add experiments to compare our algorithm HDRRM against the MDRMS\cite{asudeh2017efficient} algorithm for the regret-ratio minimization set (RMS) problem. In experiments, HDRRM always has the lowest rank-regret. Correspondingly, MDRMS sometimes has the highest rank-regret which is more than one order of magnitude larger than HDRRM. Due to time and space constraints, we do not make comparisons with other algorithms for RMS. 
	
}

==> file/theoretic-NSConflict-xxx-mac10.16.tex <==

\section{Theoretical Property}
\label{s_theoretical} 
In this section, we introduce a few theoretical properties about RRM and RRRM, some of which play key roles in designing the algorithms proposed in this paper. 
%At first, by proving a lower bound on the rank-regret, we show that there is no algorithm for RRM with an excellent upper bound guarantee. 
At first, by proving a lower bound on the rank-regret, we show that {\color{red} there is no algorithm for RRM with an upper bound guarantee independent of the dataset size}. 
%Next, we prove that the \textit{restricted skyline} \cite{ciaccia2017reconciling} is the set of candidate tuples for the RRRM problem, but the convex hull is not. 
Next, {\color{red} we show that the \textit{restricted skyline} \cite{ciaccia2017reconciling} is the set of candidate tuples for the RRRM problem}.
Similarly, the \textit{skyline} \cite{xiao2020sampling} is the candidate set for RRM.

\subsection{Lower Bound}

For the RMS problem, there are several algorithms \cite{nanongkai2010regret, cao2017k, agarwal2017efficient, xie2018efficient} which return a fixed size set with a theoretical upper bound on the regret-ratio. And the bound has nothing to do with the dataset size $n$. Nevertheless, by proving a lower bound closely related to $n$ on the rank-regret, we show that there is no such algorithm for the RRM problem. For lack of space, the missing proofs in this paper can be found in \cite{xiao2021rankregret}. 

\begin{theorem}
	\label{t_low_bound}
	Given integers $r\ge1$ and $d\ge2$, there is a dataset $D$ of $n$ $d$-dimensional tuples such that, for any size $r$ set $S\subseteq D$, $\nabla_\mathbb{L}(S)$ is $\Omega(n/r)$. 
\end{theorem}
\begin{IEEEproof}[Proof Sketch]
	We prove it with a two-dimensional dataset, whose tuples evenly lie on a quarter-arc in the first quadrant, with radius $1$ centered at the origin, shown as black dots in 
	%Figure \ref{fig-lower_bound}.
	{\color{red} Figure \ref{fig-lower_bound}.}
\end{IEEEproof}
%\begin{IEEEproof}
	%First, assume $d=2$. Our construction is inspired by Nanongkai et al. \cite{nanongkai2010regret}. We define the angle of a tuple/point $t$ to be $\arctan\frac{t[2]}{t[1]}$. Let $D$ be the size $n$ set $$ \{t_\theta = (\cos\theta, \sin\theta)\ |\ \theta\in\{0, \frac{\pi}{2(n-1)}, \cdots, \frac{(n-1)\pi}{2(n-1)}\}\}. $$ All tuples (black dots in Figure \ref{fig-lower_bound}) lie on a quarter-arc in $\mathbb{R}^2_+$ with radius $1$ centered at the origin. Then the angle of $t_\theta$ is $\theta$. Each tuple in $D$ is the highest utility tuple for some vectors in $\mathbb{L}$. Consider a size $r$ set $S\subseteq D$. Let the angles of tuples in $S$ are $\vartheta_1 < \vartheta_2 <\cdots < \vartheta_r$. Let $\vartheta_0=0$ and $\vartheta_{r+1}=\pi/2$, i.e., $t_{\vartheta_0}=(1,0)$ and $t_{\vartheta_{r+1}}=(0,1)$. Let $p$-$O$-$q$ be the angle subtended between lines obtained by joining the origin $O = (0, 0)$ with two points $p$ and $q$. Consider angles $t_{\vartheta_i}$-$O$-$t_{\vartheta_{i+1}}$ for all $i\in\{0,\cdots, r\}$. Note that the sum of these $r+1$ angles is exactly $\pi/2$. Therefore, at least one angle is no less than $\frac{\pi}{2(r+1)}$. Let the angle be $t_{\vartheta_i}$-$O$-$t_{\vartheta_{i+1}}$. The difference between angles of two adjacent tuples in $D$ is $\frac{\pi}{2(n-1)}$. Thus there are $\Omega(n/r)$ tuples in $D$ whose angles are larger than $\vartheta_i$ but less than $\vartheta_{i+1}$. If $i\in [r-1]$, then set $\alpha=\frac{\vartheta_i+\vartheta_{i+1}}{2}$ and consider the utility vector $u=(\cos\alpha, \sin\alpha)$. Note that the utility of each tuple $t\in D$ based on $u$ is the $L_2$-distance between the origin $O$ and the projection of $t$ onto line $O$-$(\cos\alpha, \sin\alpha)$. And the tuples in $D$ whose angles lie between $\vartheta_i$ and $\vartheta_{i+1}$ have utilities larger than those of $t_{\vartheta_i}$ and $t_{\vartheta_{i+1}}$, i.e., outrank $t_{\vartheta_i}$ and $t_{\vartheta_{i+1}}$ based on the utility vector $u$. See Figure \ref{fig-lower_bound}. In addition, $t_{\vartheta_i}$ and $t_{\vartheta_{i+1}}$ are the top-2 tuples of $S$ for $u$. Thence the rank-regret of $S$ for $u$ is $\Omega(n/r)$. If $i = 0$, then set $\alpha=0$. If $i = r$, set $\alpha=\pi/2$. With the same analysis, $\nabla_u(S)$ is also in $\Omega(n/r)$, and so is $\nabla_\mathbb{L}(S)$. 
	
	%If $d>2$, for each tuple in $D$, keep the values of first two attributes, and set those of the subsequent attributes to $1$. Then we are able to get the same result.
%\end{IEEEproof}
Therefore, for RRM, there is no algorithm whose output has an upper bound on rank-regret that is unconnected with the dataset size $n$. So does for RRRM. However, the lower bound in Theorem \ref{t_low_bound} is for the adversarial cases far from practice. 
%Algorithms proposed in this paper usually output a given size set with a constant rank-regret in experiments.
Algorithms proposed in this paper usually output a given size set with {\color{red} a small rank-regret} in experiments.

\subsection{Candidate Tuples}
Based on the restricted utility vector space $\mathbb{U}$, Ciaccia et al. \cite{ciaccia2017reconciling} proposed a new kind of dominance, through which they introduced the restricted version of skyline. 
\begin{definition}[$\mathbb{U}$-Dominance and $\mathbb{U}$-Skyline]
	Let $t$ and $t'$ be tuples in $D$, and $\mathbb{U}\subseteq\mathbb{L}$ be a set of utility vectors. Then, $t$ $\mathbb{U}$-dominates $t'$, written $t\prec_\mathbb{U} t'$, if $\forall u\in\mathbb{U}$, $w(u,t)\ge w(u,t')$ and $\exists v\in\mathbb{U}$, $w(v,t)>w(v,t')$. The $\mathbb{U}$-skyline of $D$, denoted by $\mathrm{Sky}_\mathbb{U}(D)$, is defined as
	\vspace{-1ex} $$\mathrm{Sky}_\mathbb{U}(D) = \{ t\in D\ |\not\exists t'\in D, t'\prec_\mathbb{U} t \}.$$
\end{definition}
Notice that if $\mathbb{U}$ is the full space $\mathbb{L}$, $\mathrm{Sky}_\mathbb{U}(D)$ is equivalent to the skyline\cite{xiao2020sampling} of $D$, abbreviated as $\mathrm{Sky}(D)$. In addition, for any $\mathbb{U}\subseteq\mathbb{L}$, $\mathrm{Sky}_\mathbb{U}(D)$ is the subset of $\mathrm{Sky}(D)$. Next, we show that $\mathrm{Sky}_\mathbb{U}(D)$ is the set of candidate tuples for the RRRM problem. 

\begin{theorem}
	\label{t_skyline}
	If there is a size $r$ set $S\subseteq D$ with $\nabla_\mathbb{U}(S) = k$, then there must be a set $R\subseteq\mathrm{Sky}_\mathbb{U}(D)$ such that $|R| \le r$ and $\nabla_\mathbb{U}(R) \le k$.
\end{theorem}
%\begin{IEEEproof}
	%For each tuple $t\in S$, if $t\notin\mathrm{Sky}_\mathbb{U}(D)$, there must be a tuple $t'\in\mathrm{Sky}_\mathbb{U}(D)$ such that $t'$ $\mathbb{U}$-dominates $t$. For each $u\in\mathbb{U}$, $t'$ outranks $t$. Then replace all such $t$ in $S$ with $t’$, and obtain the set $R$. By definition, for each $u\in\mathbb{U}$, $\nabla_u(R)\le\nabla_u(S)$. Thus we have $\nabla_\mathbb{U}(R) \le k$. Further, $R$ is no larger than $S$. 
%\end{IEEEproof}

The above theorem suggests that it is sufficient to focus on all subsets of $\mathrm{Sky}_\mathbb{U}(D)$ to find the solution of RRRM, and we can regard only the $\mathbb{U}$-skyline tuples as candidates. Similarly, $\mathrm{Sky}(D)$ is the candidate set for RRM. {\color{red} But in \cite{xiao2021rankregret} we prove that the convex hull \cite{asudeh2019rrr} of $D$ does not have the above property.}
%The convex hull \cite{asudeh2019rrr} of $D$, denoted by $\mathrm{Conv}(D)$, is a subset of $\mathrm{Sky}(D)$ and contains the top-1 tuple for any vector in $\mathbb{L}$. But we can show that $\mathrm{Conv}(D)$ does not have the above property. 
%\begin{theorem} \label{t_convex_not_cand} There is an input to the RRM problem such that the optimal solution is not the subset of $\mathrm{Conv}(D)$, i.e., contains a tuple not in $\mathrm{Conv}(D)$. \end{theorem}
%\begin{IEEEproof} Consider a running example as shown in Figure \ref{fig-convex}. Dataset $D$ has 7 tuples, namely $t_1, t_2, \dots, t_7$, in a two-dimensional space where the first dimension is $A_1$ and the second dimension is $A_2$. We know that when $r=1$, the optimal solution of the RRM problem is $\{t_3\}$. Note that $\mathrm{Conv}(D)$ is $\{t_1, t_2, t_4, t_5\}$ but $t_3$ is not in $\mathrm{Conv}(D)$. \end{IEEEproof}
%The result in Theorem \ref{t_convex_not_cand} is directly applicable to RRRM.


\begin{figure}[tbp]
	\centering
	\color{red}
	\begin{minipage}[htb]{0.32\linewidth}
		\tabcaption{Example} 
		\centering
		\label{tab_example}
		\scriptsize
		\begin{tabular}{c|l|l}
			& $A_1$ & $A_2$ \\ \hline
			$t_1$ & 0 & 1 \\ \hline
			$t_2$ & 0.4 & 0.95 \\ \hline
			$t_3$ & 0.57 & 0.75 \\ \hline
			$t_4$ & 0.79 & 0.6 \\ \hline
			$t_5$ & 0.2 & 0.5 \\ \hline
			$t_6$ & 0.35 & 0.3 \\ \hline
			$t_7$ & 1 & 0
		\end{tabular}
	\end{minipage}
	\begin{minipage}[htb]{0.32\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{figures/fig-example.png} 
		\caption{Null}
		\label{fig-example}
	\end{minipage}
	\begin{minipage}[htb]{0.32\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{figures/fig-shift.png} 
		\caption{Null}
		\label{fig-shift}
	\end{minipage}
	\vspace{-3ex} 
\end{figure}

\begin{figure*}[tbp]
	\centering
	\color{red}
	\begin{minipage}[htb]{0.18\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{figures/fig-lower_bound.png} 
		\caption{Proof Idea of Theorem \ref{t_low_bound}}
		\label{fig-lower_bound}
	\end{minipage}
	\begin{minipage}[htb]{0.18\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{figures/fig-dual.png} 
		\caption{Dual Representation for Tuples in Figure \ref{fig-example}}
		\label{fig-dual}
	\end{minipage}
	\begin{minipage}[htb]{0.18\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{figures/fig-intersect.png} 
		\caption{Intersections between Lines}
		\label{fig-intersect}
	\end{minipage}
	\begin{minipage}[htb]{0.44\linewidth}
		\tabcaption{updates of $M$} 
		\centering
		\label{tab_m}
		\begin{tabular}{c|l|l|l|l}
			& Initial & $(l_1,l_2)$ & $(l_1,l_3)$ & $(l_2,l_3)$\\ \hline
			$M[1,1]$ & $\{l_1\}$,1 & -,2 & -,3 & -,- \\ \hline
			$M[1,2]$ & $\{l_1\}$,1 & -,2 & -,3 & -,- \\ \hline
			$M[2,1]$ & $\{l_2\}$,2 & -,- & -,- & -,- \\ \hline
			$M[2,2]$ & $\{l_2\}$,2 & $\{l_1,l_2\}$,1 & -,- & -,2 \\ \hline
			$M[3,1]$ & $\{l_3\}$,3 & -,- & -,- & -,- \\ \hline
			$M[3,2]$ & $\{l_3\}$,3 & -,- & $\{l_1,l_3\}$,2 & -,-
		\end{tabular}
	\end{minipage}
\vspace{-3ex} 
\end{figure*}

==> ref/HDref.tex <==
\section{HD Algorithm Reference}

RRR

In high-dimensional cases (HD) where $d>2$, the continuous function space becomes problematic, the geometric shapes become complex, and even the operations such as computing the volume of a shape and the set operations become inefficient. Therefore, in this section, we use the k-set notion [17] to take an alternative route for solving the RRR problem by transforming the continuous function space to discrete sets. This leads to the design of an approximation algorithm that guarantees the rank-regret of k, introduces a log approximation-ratio in the output size, and runs in polynomial time, for a constant number of dimensions.

21PODS

Although representing the approximate Voronoi cells and performing set operations on Voronoi cells are hard in $\mathbb{R}^d$ when $d\ge 3$, determining the membership of a vector $u$ in $V^k_{\mathbb{S},t}$ for a tuple $t$ is much easier. Specifically, given a vector $u\in\mathbb{S}$, a tuple $t\in T$, and an integer $k\in[1,n]$, we have $u\in V^k_{\mathbb{S},t}$ if and only if $M(u,t)\le k$. So it is possible to discretize Voronoi cells by sampling a set of vectors on $\mathbb{S}$ and performing the membership tests for all vectors w.r.t. each tuple. In this way, we can approximately represent $V^k_{\mathbb{S},t}$ by the subset of vectors in it. Intuitively, the more vectors we use, the smaller the resulting error.

SIGMOD2017

We introduce a conceptual model of the problem as an infinitely large matrix min-max problem [24]. We “operationalize” such a conceptual model with a matrix discretization approach that provides a user-controllable discretization parameter. After discretizing the problem space to a manageable size, we then construct a reduction to set-cover [12] which solves the min-max problem deterministically in (theoretically) O(nlogn) time, while guaranteeing a regret-ratio within any arbitrarily small user-controllable distance from the optimal regret-ratio. We make this algorithm more practical by incorporating an existing approximation algorithm for set-cover. Our final algorithm outperforms existing solutions by an order of magnitude over real-world datasets, as we shall show in the experimental evaluations.

SEA2017

In this section, we present an efficient scheme to approximate the optimal k-regret set, by formulating the RMS problem as a hitting-set problem. A range space (or set system) S = (X, R) consists of a set X of objects and a family R of subsets of X. A subset $H\subseteq X$ is a hitting set of S if H R =  for all R in R. The hitting set problem asks to compute a hitting set of the minimum size. The hitting set problem is a classical NP-Complete problem, and a well-known greedy O(log n)-approximation algorithm is known.

We construct a set system S = (P, R) such that a subset Q $\subseteq$ P is a (k)-regret set if and only if Q is a hitting set of S. We then use the greedy algorithm to compute a small-size hitting set of S. A weakness of this approach is that the size of R could be very large and the greedy algorithm requires R to be constructed explicitly. Consequently, the approach is expensive even for moderate inputs say d = 5.

Inspired by the above idea, we propose a bicriteria approximation algorithm: given P and e > 0, we compute a subset QP of size O(s log s) that is a (k,2)-regret set of P; the constant 2 is not important, it can be made arbitrarily small at the cost of increasing the running time. By allowing approximations to both the error and size concurrently, we can construct a much smaller range space and compute a hitting set of this range space.

We first show how to formulate the min-size version of the RMS problem as a hitting set problem. Let P, k, and e be fixed. For a vector u in X, let Ru = {p in P | w(u, p) >= (1-e)wk(u, p)}. Note that if e = 0, then Ru = Sk (u), the set of top-k points of P in direction u. Set Ru = {Ru | u in X}. Although there are infinitely many preferences we show below that |Ru| is polynomial in |P|. We now define the set system S = (P, Ru ).

We can thus compute a small-size (k)-regret set of P by running the greedy hitting set algorithm on S. In fact, the greedy algorithm in [7] returns a hitting set of size O(slogs). As mentioned above, the challenge is the size of Ru. Next, we show how to construct a much smaller set system. Let N be a 2d-net of U, and let RN = {Ru | u in N}. Set SN = (P, RN ). Our main observation, stated in the lemma below and proven in Appendix B, is that it suffices to compute a hitting set of SN . Recall that basis B of P is the subset of at most d points, one per coordinate, corresponding to the points with the highest value per coordinate.

%PODS2021
%In this section, we introduce the Voronoi diagrams [9], from which we can draw geometric insights for the MC problem and build the theoretical foundation of our proposed algorithms. A Voronoi diagram for a point set  P is defined in terms of a similarity measure, which is the inner product function here. Prior work has investigated the relationships between the inner-product Voronoi diagram and graph-based maximum inner product search [32, 36, 42]. We will first consider using the inner-product Voronoi diagram for coreset construction in this work.
%Formally, for a point set P, its Voronoi diagram is a collection of Voronoi cells, one defined for each point p in P. The Voronoi cell R(p) of point p is defined as the set of unit vectors for which p is the maximum. By definition, a point p is an extreme point if and only if its Voronoi cell is non-empty. It is also not difficult to see that the set of extreme points consists exactly of the set of vertices of the convex hull of P.
%To illustrate MC geometrically, we extend the notion of Voronoi cells to approximate Voronoi cells. Specifically, the approximate Voronoi cell of point p is defined as the set of unit vectors for which the inner product of p is within an approximation to the maximum of P. Equivalently, the loss in the maxima of Q w.r.t. P is at most for any vector in. So, from a geometric perspective, MC can be regarded as the set cover problem of finding the minimum subset of points from P such that the union of their approximate Voronoi cells is S.

ICDE2020

In general, the utility functions in FC could have an arbitrary distribution. For the ease of presentation, we first assume that each utility function in FC is equally probable to be used by a user. However, we will later relax this assumption in Section IV-C2 and show that our techniques can be easily applied when arbitrary types of distributions are considered.

Intuitively, given a point p in D, the (uncountable) number of utility functions in Fp can be regarded as the importance of p. A point with a higher importance indicates that this point has the maximum utility w.r.t. more utility functions. Based on this observation, our algorithm has two major steps. 
Firstly, we compute the function set Fp for each p in D and quantify its importance. Secondly, we leverage a greedy algorithm to select points to S according to the importance obtained in the first step until $\sum Fp = FC$. In the following, we first present the formal definition of Fp and then provide the procedure for computing the desired Fp.

In Section III, Fp is defined to be a set of utility functions, whose utility vectors are in Cone(Ext(p), O). In other words, Fp can be represented as a partial spherical surface of S, i.e., $Cone(Ext(p), O)\cup S$. With a slight abuse of terminology, when S is clear in the context, we also call the spherical surface $Cone(Ext(p), O)\cup S$ as the conical hull of p, denoted by Cp . Clearly, Cp is also uniquely defined by Ext(p). Intuitively, if there are more vectors in Cp , p is more important since it has the maximum utility w.r.t. more functions. 
However, since the number of vectors in Cp is uncountable, we use the “surface area” (i.e., the (d-1)-dimensional measure) to quantify the importance of a point p. Specifically, we define the volume of a conical hull of p (or simply, the volume of p), denoted Area(C ) p by Vol(p), to be Area(S) , where Area(·) denotes the surface area. The volume of a set S, denoted by Vol(S). It is easy to see that Vol(S) in [0, 1]. The following lemma shows that our goal of finding a set S with $\sum Fp = FC$ is equivalent to finding a S with Vol(S) = 1.

To find the desired set S with Vol(S) equal to 1, a crucial operation is to compute Vol(S) for a given S. We first treat the computation of Vol(S) as a black box and present a conceptual algorithm in Section IV-B. Since the exact (actual) volume Vol(S) is time-consuming to compute especially in a high dimensional space, we present an algorithm which utilizes the approximate (estimated) volume Vol(S) in Section IV-C.

Unfortunately, computing the exact value of Vol(S) (which is not necessarily convex) is very expensive especially in a high dimensional space. Thus, we utilize a sampling method to estimate the (marginal) volume of a conical hull. Specifically, given a Fp, we generate N unit samples from R+d by a d-dimensional uniform distribution and determine the number of samples inside this Fp. Then, the volume of this conical hull is estimated to be the ratio of the number of samples locating inside the conical hull to the total number of samples, N.

Algorithm can also be interpreted in a set-cover manner. We say that a sample s is covered by a conical hull Cp  if s lies inside Cp . The greedy algorithm starts with an empty solution set S, and it adds points to S iteratively until all samples are covered by some conical hulls corresponding to the points in S. In each iteration, it adds the point whose conical hull covers the largest number of uncovered samples (i.e., the point with the largest estimated marginal volume).

==> ref/exper.tex <==

\section{Experiment Reference}

In some plots there are missing values for the CTVW algorithm, because we stopped the execution after running it on a data set for 2 days.

RRR

We also implemented the k-set graph based enumeration for MD. We did not include the results here, but we observed that it does not scale beyond \textbf{a few hundred items} (that is because it need to solve much as O(nk) linear programs for a single k-set). Instead, we apply the randomized algorithm k-setr for finding the k-sets (while setting the termination condition c to \textbf{100}).
However, in their practical implementations, the value $c$ is determined empirically.

Still, because the sweeping ray algorithm(2DRRR) is quadratic, these algorithms did not scale beyond \textbf{100K} items.

Although significantly smaller than the upper bound, still the sizes are large enough to make the k-set discovery mpractical for large settings. For example, running the k-setr algorithm for the DOT dataset and $k = 10\%$ took more than \textbf{ten thousand seconds}. 

MDRC uses the fact that the k-sets are highly overlapping and recursively partitions the space into several hypercubes and stops the recursion for each hypercube as soon as the intersection of the top-k items in its corners is not empty.

Looking at these figures, first \textbf{MDRRR} did not scale for \textbf{100K} items. The reason is that mdrrr needs the collection of k-sets in order to apply the hitting set. For a very large number of items even the k-setr algorithm does not scale.


SIGMOD17

\textbf{Fixed Without Dimension. }
Given the importance of the choice of $m$, we evaluate the impact of the sample size in the following section. On examining the experiment results, it turns out even though increasing the value $m$ increases the running time significantly, the improvement on the quality of results drops quickly. In our experiments, choosing $m$ between $1000$ and $10000$ seemed to be appropriate.

Impact of the discretization control parameter (gamma): Figures 24, 25, and 26 show the performance of the algorithms for correlated, independent, and anti-correlated datasets respectively. Increasing the value of gamma highly affects on the performance(regret ratio) of the HD-RRM algorithm. On the other hand, increasing the value of gamma directly affects on the running time of the algorithms. Looking at the figures, at least in these experiments, selecting gamma between 4 and 6 seems appropriate, as it seems to reach a point of saturation where increasing gamma benefits little in terms of execution time.

VLDBJ20

\textbf{Anti-correlated datasets} are the most interesting synthetic datasets where the skyline set is large and cannot be returned as a whole. Thus, we used anti-correlated datasets as our default synthetic datasets. 

The performance of each algorithm is measured by its query time and maximum rank-regret.

SIGMOD21

Identifying Insufficient Data Coverage for Ordinal Continuous-Valued Atributes. 

\textbf{the adversarial case not happen; adjacent k-sets are similar; DOUBLE. }
Specifically, we use an exponential search strategy: starting from an initial value for the number of samples, we iteratively double the number of samples until we ind a proper number of samples.

PODS21

\textbf{DOUBLE. }
Since the sampling complexities of ANN and SCMC increase exponentially with d and thus become impractical for a large d, we adopt an alternative sampling strategy: Rather than performing the sampling all at once, we sample them in stages and maintain a coreset Q until $regret(Q) <= e$.

ICDE21

\textbf{Binary Search. }
Since e-KERNEL and HS are proposed for min-size k-RMS that returns the smallest subset whose maximum k-regret ratio is at most e, we adapt them to our problem by performing a binary search on e in the range (0, 1) to find the smallest value of e that guarantees the result size is at most r.

SEA17

\textbf{DOUBLE. code}
Sample size for verification is different for different dimensions. 
RRS is the Randomized Regret Set algorithm, based on coresets, described in Section 3.1 In our implementation, rather than choosing O((d-1)/2 ) random preferences all at once, we choose them in stages and maintain a subset Q until $regret(Q) <=e$.
HS is the Hitting Set algorithm presented in Section 4. Furthermore, instead of choosing O(d-1) directions in one step and find a hitting set, we can sample in stages and maintain a hitting set until we find a (k,e)-regret set.
In evaluating the quality $regret_k(Q)$ of a regret set Q, we compute the regret for a large set of random preferences (for example for d = 3 we take 20000 preferences), and use the maximum value found as our estimate. In fact, this approach gives us the distribution of the regret over the entire set of preference vectors.


ALENEX18

\textbf{DOUBLE. }
For a certain number m, we start by taking m points on the unit sphere. Let S be that sample set. As in [1], for each s in S we add in P' the point p in P such that p = nn(s, P), where nn(s, P) is the nearest neighbor of s in the set P. 
We then check if P' is a (1,e)-kernel by testing using a large set of directions V if the set P' satisfies the conditions of being a (1,e)-kernel. 
If yes, we stop and output P'. Otherwise, we repeat the sampling process and the nearest-neighbor queries taking 2m samples, and so on.

ICDE20

\textbf{FIXED. }
Unless stated explicitly, for each synthetic dataset, the sampling size is set to be 10,000 (i.e., N = 10, 000). 
Note that theoretically, both CORESET and CORESETHS in ALENEX18 have to sample (much) utility functions to construct the solutions. However, in their practical implementations, the number of utility functions they sampled is determined empirically (i.e., a number much smaller than theoretical). We follow this setting and use the reported parameters in [13] in our experiments.

Some results are plotted in log-scale for better visualization.

We also studied the effect of our sampling strategy by varying the sampling size N (and set alpha to be 0.99, the default value). The results on a 3-dimensional dataset are shown in Table IV. When N is very small, minHap (S) can be less than (but close to) alpha; for example, we can achieve a 0.98 happiness ratio with only 100 samples. When N becomes larger (i.e., becomes smaller), the estimated volume is closer to the actual volume and thus, minHap (S) becomes closer to alpha.
In particular, when N >= 5000, the returned set S achieves the required happiness level 0.99 and its size becomes stable, i.e., the size does not increase further with more sampling points. Compared with the competitors which achieve the same happiness level, CONE-GREEDY outputs the smallest number of points. Note that a large sampling size N is useful in achieving the required happiness ratio, but it can introduce additional time. On the other hand, a small N results in a faster algorithm but it can also give a large error in the estimated volume. Following the practical way of determining the sampling size in CORESET and CORESETHS, we set the default sampling size to be 10000 in our experiments since it achieves a reasonable trade-off between the efficiency and the effectiveness according to the results in Table IV. 



RRR experiment

The MD algorithms proposed in § 5 are the hitting-set based algorithm mdrrr and the space function covering algorithm mdrc. 

the space partitioning algorithm mdrc. 

MDRC-On the other hand mdrc does not depend on finding the k-set or sweeping a line. Rather, it partitions the space until top-k of two corners of each range intersect. Due to the binary search nature of the algorithm that breaks the space by half at every iteration, soon the functions in the two ends of each range become similar enough to share an item in their top-k. Therefore, the algorithm performs very well in practice, and scales well for large settings. 

MDRC-Given the possibly large number of k-sets and the cost of finding them (even using the randomized algorithm k-set r ), MDRC is designed to prevent the k-set enumeration. mdrc uses the fact that the k-sets are highly overlapping and recursively partitions the space (see Figure 8) into several hypercubes and stops the recursion for each hypercube as soon as the intersection of the top-k items in its corners is not empty. This algorithm performs very well in practice, as after a few iterations, the functions in the corners become similar enough to share at least one item in their top-k. 

MDRC-has the least running time for large values of n and in all cases it finished in less than a few seconds. The reason is that after a few recursions, the functions in the corners of the hypercubes become similar and share an item in their top-k.

MDRC-One interesting fact in these plots is that the running time of mdrc decreases as k increases. This is despite the fact that, , the number of k-sets increased. The probability that the top-k of corners of a hypercube share an item increases when looking at larger values of k where each set contains more items.  

k-set-First, as observed in the figures, the actual sizes of the k-sets are significantly smaller than the best known theoretical upper-bound for 3D. In fact, the number of k-sets is closer to n than the upper-bounds. Recall that the k-sets are densely overlapping, as the neighboring k-sets in the k-set graph only differ in one item. As k increases (up until k = 50), for each node of the k-set graph the number of candidate transitions to the neighboring k-sets increases which affect |S| as well.Although significantly smaller than the upper bound, still the sizes are large enough to make the k-set discovery impractical for large settings. 

MDRRR-is the hitting set based algorithm that, given the collection of k-sets, guarantees the rank-regret of k and a logarithmic increase in the output size. 

MDRRR-Looking at these figures, first mdrrr did not scale for 100K items. The reason is that mdrrr needs the collection of k-sets in order to apply the hitting set. For a very large number of items even the K-SET$_r$ algorithm does not scale. 

MDRRR-since the hitting set based algorithm mdrrr requires the collection of k-sets, it was not efficient. 

MDRRR- had the worst performance, and it got worse as k increased. The bottleneck in mdrrr is the k-set enumeration, and it increased by k, as the number of k-sets increased. 






==> ref/intro.tex <==

\subsection{Introduction Reference}

Abstract-Selecting the best items in a dataset is a common task in data exploration. However, the concept of “best” lies in the eyes of the beholder: different users may consider different attributes more important, and hence arrive at different rankings. Nevertheless, one can remove “dominated” items and create a “representative” subset of the data set, comprising the “best items” in it. A Pareto-optimal representative is guaranteed to contain the best item of each possible ranking, but it can be almost as big as the full data. Representative can be found if we relax the requirement to include the best item for every possible user, and instead just limit the users’ “regret”. Existing work defines regret as the loss in score by limiting consideration to the representative instead of the full data set, for any chosen ranking function. However, the score is often not a meaningful number and users may not understand its absolute value. Sometimes small ranges in score can include large fractions of the data set. In contrast, users do understand the notion of rank ordering. Therefore, alternatively, we consider the position of the items in the ranked list for defining the regret and propose the rank-regret representative as the minimal subset of the data containing at least one of the top-k of any possible ranking function.

Randomized enumeration(K-SET$_r$): The sizes are large enough to make the k-set discovery impractical for large settings. First, mdrrr based on K-SET$_r$ did not scale for 100K items. The bottleneck in mdrrr is the k-set enumeration. 
Recall that the k-sets are densely overlapping, as the neighboring k-sets in the k-set graph only differ in one item. As k increases (up until $k = 50\%$), for each node of the k-set graph the number of candidate transitions to the neighboring k-sets increases which affect $|S|$ as well.

Score vs Rank: The actual scores assigned by the functions are usually made up and do not carry a significant meaning. Furthermore, there might even be a non-linearity in the raw attribute values themselves. That is, uniform changes in attribute values may not uniformly change the “quality” of an item with that value. These motivate the rank difference as an alternative for defining the measure of regret.

SIGMOD17-We develop an approximation algorithm that runs in linearithmic time and guarantees a regret ratio, within any arbitrarily small user-controllable distance from the optimal regret ratio. We develop HD-RRM, an algorithm for higher dimensions that can approximate the regret ratio to within a user controlled parameter. This issue inspires us to develop a linearithmic approximate solution that offers a guaranteed approximation ratio adjustable by a user-controlled parameter. 

ICDE2014-Consider the following example. Assume that we have a database storing a multitude of cars, each of which is associated with two attributes, namely, horse power (HP) and miles per gallon (MPG). Suppose that Alice wants to buy a car with high HP and high MPG. Since the size of a car database is usually very large (e.g., over 350,000 cars in the database of www.autotrader.co.uk), the database system selects a small number of cars from the database based on a certain criterion and displays them to Alice.

ICDE2020-Consider the following car database application. Assume that Alice attempts to buy a car from a car database where each car is represented by two attributes, namely horse power (HP) and miles per gallon (MPG). To assist Alice for making the decision, she should be provided with cars that she is potentially interested in (e.g., cars with high utilities if we know Alice’s utility function). However, in practice, it is difficult for Alice to provide her utility function explicitly (hence, we cannot use a top-k query). Alternatively, we can approach this problem as RRM query: Alice specifies a size bound (which is easier for her to do), which represents the largest number of cars she expects to look through. In practice, Alice can set size bound to be at most 10. Then, a RRM query returns a set of tuples from the database, with size is at most 10, so that Alice will be satisfied with the returned set (since the rank-regret is as small as possible).

In practical scenarios, users are interested in achieving low rank-regret in RRM queries. For example, when buying a car/house, which is one of the big purchases in our life, a user may want to find a car/house which is as close to his/her ideal one as possible by only examining a few options. Otherwise, the user might feel regretful (i.e., not happy) for not buying a better one for a long time. Solutions of smaller sizes effectively makes the user’s decision easier.

==> ref/m.tex <==
\section{Real Value of Sample Size}
\textbf{Distance.Old by Sampling.}
$\mathbb{S}\subseteq[0,1]^d$. Consider $d$ ge $(d-1)$-dimensional up-facet, for example, $\{u\in[0,1]^d\ |\ u[1]=1\}$. partitioning each of the $d$ up-facets into $h^{d-1}$ $(d-1)$-dimensional “hypercubes” of diameter $\delta$ where $h$ is computed to be $\sqrt{d-1}/\delta$, i.e., $(d-1)\times(1/(\frac{\sqrt{d-1}}{\delta}))^2=\delta$. Then the total number of hypercubes is $num=dh^{d-1}=d(\frac{\sqrt{d-1}}{\delta})^{d-1}$. Based on the coupon collection problem and Markov's inequality, with probability at least $1-1/c$, using $c\times num\ln(num)$ samples is enough to "hit" all hypercubes, i.e., a uniform random set of $cd(\frac{\sqrt{d-1}}{\delta})^{d-1}\times(\ln d+(d-1)\ln\frac{\sqrt{d-1}}{\delta})$ vectors in $\mathbb{S}$ is a $\delta$-net of $\mathbb{S}$ with probability at least $\frac{1}{c}$. $\epsilon = \frac{2d\delta}{1+2d\delta}$, then $\delta>\epsilon/2d$. 

$$m < cd(\frac{2d\sqrt{d-1}}{\epsilon})^{d-1}\times(\ln d+(d-1)\ln\frac{2d\sqrt{d-1}}{\epsilon}). $$

if $c=1, d=3, \epsilon =0.1$, then $m\le215577$. 
$d=4$, then $m\le172186147$. \textbf{Dimensional explosion}.




==> ref/rrrm.tex <==

\subsection{RRRM Reference}
R-Skyline---p-skyline allows no \textbf{1st-trade-off} between attributes.R-skylines can take into account the different importance that different attributes might have. R-skylines may be used to model priority by means of arbitrary constraints on the space of the weights, thus allowing for more flexibility. Overall, this leads to the novel concept of \textbf{F-dominance}, in which a tuple t F-dominates tuple s when t is always better than or equal to s according to all the scoring functions in F (and strictly better for at least one scoring function in F).

SIGMOD18---In practice, however, user preferences (weights) may only be estimated with bounded accuracy, or may be inherently uncertain due to the inability of a human user to specify exact weight values with absolute accuracy. Given uncertain preferences, that is, an approximate description of the weight values. The weight vector w represents the user’s preferences, and thus is key in producing useful recommendations. Usually, it is assumed to be input directly by the user. Alternatively, it may be mined from the user’s past choices/behavior [28, 9, 27, 33], estimated by having the user make pairwise comparisons for a number of testing pairs of alternatives [26, 41], etc. 
Our work is motivated by the crucial role of \textbf{weight accuracy} in the practicality and usefulness of the top-k query. We argue that, the assumption/requirement that the exact weight vector is known is hardly realistic. Be it specified directly by the user or by a preference learning algorithm, it is inherently inaccurate. Instead, it would be wiser if user inputs were dealt with as mere indications, and a leeway were given for inaccuracies in weight setting. Similarly, in preference learning techniques, the computed weight vector should only be used as a rough guide, rather than taken as an exact representation of user preferences. \textbf{A} natural way to deal with this issue, and offer a more user-centric and practical design, is to expand the (explicitly input or computationally learned) weight vector into a region. 
The third input to UTK is a region R in preference domain. For ease of presentation, we assume that it is an \textbf{axis-parallel hyper-rectangle}, yet our techniques apply directly to general \textbf{convex polytopes}.

Marrying Top-k---The dominance paradigm is not \textbf{2nd-personalizable}, reporting the same result for every user. Personalization (i.e., serving the specific preferences of an individual user) is a hard requirement for decision support, especially nowadays, when large amounts of personal information are available via smartphones, fitness trackers, online activities, etc. Ranking by utility, in the form of a top-k query, is both personalized and OSS. 
Its Achilles’ heel, however, lies in specifying the \textbf{“correct”} weights, since a small change in w can drastically alter the top-k result [39, 80]. Vector w is assumed to be either input directly by the user or somehow mined (e.g., via online behavior and review mining [41, 71], pairwise comparisons of example records [40, 60], or some other preference learning technique [24]). In the former case, a user cannot be reasonably expected to quantify with absolute precision the relative importance of the various attributes. In the latter, preference learning methods come with an understanding that the mined w is only an estimate. This shortcoming motivates a third hard requirement for practical decision support, which is relaxed preference input, i.e., some flexibility in the specified preferences.
Ciaccia and Martinenghi [20] define that r \textbf{R-dominates} t if r scores higher than t for any w in R. They compute the R-skyline (i.e., the records that are not R-dominated by any other) by integrating that test into standard skyline algorithms. Mouratidis and Tang [54] extend potential optimality to k >= 1, i.e., they identify the records that appear in the top-k result for at least one w in R. The user/application cannot determine (or even predict) the size of the output. 

Eclipse-What is desired here is the customizability on the \textbf{3rd-“breadth”} of the attribute weights which can capture a user’s rough preference among the attributes. Intuitively, the range of [l, h] for the attribute weight ratio allows users to have a customizable and approximate preference of the relative importance of the attributes rather than an exact value l (as in 1NN) or an infinite interval [0,n) (as in skyline). For practical usage, in order to reduce the burden of parameter selection for users, we envision that users can either specify an attribute weight vector as in kNN which can be relaxed into ranges with a margin. 

Mine-Some utility vectors are rarely used by users. In addition, limiting the utility vector space can make the rank-regret of the result smaller.
